Multimodal Masked Autoencoders Learn Transferable Representations

Building scalable models to learn from diverse, multimodal data remains an open challenge. For vision-language data, the dominant approaches are based on contrastive learning objectives that train a separate encoder for each modality. While effective, contrastive learning approaches introduce sampling bias depending on the data augmentations used, which can degrade performance on downstream tasks. Moreover, these methods are limited to paired image-text data, and cannot leverage widely-available unpaired data. In this paper, we investigate whether a large multimodal model trained purely via masked token prediction, without using modality-specific encoders or contrastive learning, can learn transferable representations for downstream tasks. We propose a simple and scalable network architecture, the Multimodal Masked Autoencoder (M3AE), which learns a unified encoder for both vision and language data via masked token prediction. We provide an empirical study of M3AE trained on a large-scale image-text dataset, and find that M3AE is able to learn generalizable representations that transfer well to downstream tasks. Surprisingly, we find that M3AE benefits from a higher text mask ratio (50-90%), in contrast to BERT whose standard masking ratio is 15%, due to the joint training of two data modalities. We also provide qualitative analysis showing that the learned representation incorporates meaningful information from both image and language. Lastly, we demonstrate the scalability of M3AE with larger model size and training time, and its flexibility to train on both paired image-text data as well as unpaired data.

==> tex/backup.tex <==
\begin{table}[!htbp]
\centering
\begin{tabular}{llll}
\hline
Epochs         & 25   & 50   & 100  \\ \hline
\ours{} & 62.9 & 64.1 & 64.8 \\ \hline
MAE & 47.8 & 50.1 & 55.2 \\ \hline
\end{tabular}
\caption{
ViT-L/16 with longer pre-training schedules (25/50/100 epochs).
}
\label{tab:epochs}
\end{table}


\begin{table}[!htbp]
\centering
\begin{tabular}{llll}
\hline
Model         & ViT-S   & ViT-B   & ViT-L  \\ \hline
\ours{} & 38.2 & 58.2 & 64.1 \\ \hline
MAE & 32.1 & 44.2 & 50.1 \\ \hline
\end{tabular}
\caption{
Comparing ViT model variants of different capacities (ViT-S/B/L). All models are pre-trained for 100 epochs.
}
\label{tab:model}
\end{table}


\begin{table}[!htbp]
\centering
\begin{tabular}{llll}
\hline
& CLIP & MAE  & \ours{} \\ \hline
\begin{tabular}[c]{@{}l@{}}Linear CLS  \end{tabular} & 69.0 & 45.2 & 59.4 \\ \hline
\end{tabular}
\caption{ImageNet result. All models (ViT-B) are pre-trained for 100 epochs on CC12M~\citep{changpinyo2021conceptual}. 
}
\label{tab:linear}
\end{table}


\begin{table}[!htbp]
\centering
\begin{tabular}{lllll}
\hline
Text mask ratio         & 0.90   & 0.75   & 0.50 & 0.15 \\ \hline
\ours{} & 62.6 & 64.1 & 62.5 & 53.3 \\ \hline
\end{tabular}
\caption{
Comparing \ours{} with different text mask ratio. All models ViT-L pre-trained for 50 epochs.
\HL{XG: }
}
\label{tab:text_ratio_ablation}
\end{table}


% Following the MAE~\citep{he2021masked}, we evaluate the image encoder robustness on several widely used downstream datasets, such as ImageNet-Corruption, ImageNet-Adversarial, etc. 

% \TODO{I'm not sure what this means?}
% To conduct a fair comparison, the metric and division for each dataset that can be collected are consistent with those of MAE. 

% \begin{wrapfigure}[18]{r}{.45\textwidth}
% \begin{minipage}{\linewidth}
% \begin{figure}
%     \centering
%     \begin{subfigure}
%         \includegraphics[width=\textwidth]{figs/mixed_data.pdf}
%         % \vspace{-\intextsep}
%         \caption{Comparison of \ours{}, MAE, and CLIP on ImageNet. \ours{} significantly outperforms MAE. \ours{} can flexibly leverage both paired image-text data and unpaired image only data.
%         All models are ViT-B. MAE and M3AE are pretrained on CC12M for 100 epochs.
%         }
%     \end{subfigure}
    
%     % \bigskip% <-- added
    % \begin{figure}{\textwidth}
    %     \begin{table}
    %     % \centering
    %     \begin{tabular}{ccc}\hline CLIP & MAE & M3AE \\ \hline \(69.0\) & \(45.2\) & \(59.4\) \\ \hline\end{tabular}
    %     \caption{ImageNet result. All models (ViT-B) are pre-trained for 100 epochs on CC12M~\citep{changpinyo2021conceptual}. 
    %     }
    %     \label{tab:linear}
    %     \end{table}
    % \end{figure}
    
%     \label{fig:mixed_data}
% \end{figure}
% \end{minipage}
% \end{wrapfigure}

==> tex/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Our paper does not contain any human experiments and all the experiments are performed on public datasets.}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code will be provided in the supplementary material.}
  \item Did you specify all the training details (\eg, data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (\eg, with respect to the random seed after running experiments multiple times)?
    \answerNA{The results are not sensitive to random seeds}
        \item Did you include the total amount of compute and the type of resources used (\eg, type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We describe the compute resources used in the applendix}
\end{enumerate}


\item If you are using existing assets (\eg, code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We used public dataset CC12M~\citep{changpinyo2021conceptual}, ImageNet~\citep{deng2009imagenet} and CIFAR~\citep{krizhevsky2009learning}}
  \item Did you mention the license of the assets?
    \answerYes{We include the license information in the appendix.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{The datasets we use are public and do not contain personally identifiable information.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tex/limitation.tex <==
One major limitation of this work is that it requires large-scale computation to pre-train and thus consumes significant energy. We hope that with the rapid progress of efficient hardware and renewable energy, this limitation can be overcome in the near future. Like any other general purpose representation learning models, our model could have both positive (\eg, enabling access to more information by improving machine translation) and negative (\eg, loss of jobs with more automation) impact on the society. These impacts are broadly applicable to pre-trained models and not specific to this work.
